Weighted Min-Cut: Sequential, Cut-Query and Streaming Algorithms

Consider the following 2-respecting min-cut problem. Given a weighted graph $G$ and its spanning tree $T$, find the minimum cut among the cuts that contain at most two edges in $T$. This problem is an important subroutine in Karger's celebrated randomized near-linear-time min-cut algorithm [STOC'96]. We present a new approach for this problem which can be easily implemented in many settings, leading to the following randomized min-cut algorithms for weighted graphs. * An $O(m\frac{\log^2 n}{\log\log n} + n\log^6 n)$-time sequential algorithm: This improves Karger's $O(m \log^3 n)$ and $O(m\frac{(\log^2 n)\log (n^2/m)}{\log\log n} + n\log^6 n)$ bounds when the input graph is not extremely sparse or dense. Improvements over Karger's bounds were previously known only under a rather strong assumption that the input graph is simple [Henzinger et al. SODA'17; Ghaffari et al. SODA'20]. For unweighted graphs with parallel edges, our bound can be improved to $O(m\frac{\log^{1.5} n}{\log\log n} + n\log^6 n)$. * An algorithm requiring $\tilde O(n)$ cut queries to compute the min-cut of a weighted graph: This answers an open problem by Rubinstein et al. ITCS'18, who obtained a similar bound for simple graphs. * A streaming algorithm that requires $\tilde O(n)$ space and $O(\log n)$ passes to compute the min-cut: The only previous non-trivial exact min-cut algorithm in this setting is the 2-pass $\tilde O(n)$-space algorithm on simple graphs [Rubinstein et al., ITCS'18] (observed by Assadi et al. STOC'19). In contrast to Karger's 2-respecting min-cut algorithm which deploys sophisticated dynamic programming techniques, our approach exploits some cute structural properties so that it only needs to compute the values of $\tilde O(n)$ cuts corresponding to removing $\tilde O(n)$ pairs of tree edges, an operation that can be done quickly in many settings.

==> cc-implement.tex <==
\subsection{2-party communication upper bound} \label{sec:cc-implement}

In the model of 2-party communication complexity, we assume that the edges of the graph $G$ is distributed (arbitrarily) between two players, Alice and Bob. We also assume that Alice and Bob both know the underlying spanning tree $T$, and their goal is to output a cut of $G$ which is minimum among all cuts which 2-respects $T$. Let us denote the tree induced by the edges that Alice holds by $G^A \subseteq G$ and that of Bob by $G^B \subseteq G$. Associated with $G^A$ (and $G^B$), there is a cost-matrix $M_{G^A}$ (and $M_{G^B}$) which Alice (and Bob resp.) can compute by herself (himself). We denote the $(i,j)$-th entry of $M_{G^A}$ (and $M_{G^B}$) as $\cost^A(i,j)$ (and $\cost^B(i,j)$ resp.). Note that $M_{G^A} + M_{G^B} = M_G$.

First, we see how Alice and Bob can compute a cut-sparsifier among themselves with little communication. 
\begin{lemma} \label{clm:cc-sparsifier}
The communication complexity of computing a cut-sparsifier is $\tO(n)$.
\end{lemma}
\begin{proof}
Note that, cut-sparsifier is linear in the following sense: If Alice computes a sparsifier $H^A$ corresponding to her graph $G^A$, and Bob computes a sparsifier $H^B$ corresponding to $G^B$, then $H = H^A \cup H^B$ is a cut-sparsifier of $G$. For any cut $S$, $C_{H^A}(S) \in (1 \pm \eps)C_{G^A}(S)$, and similarly $C_{H^B}(S) \in (1 \pm \eps)C_{G^B}(S)$. Then it is clear that \[
C_H(S) = C_{H^A}(S) + C_{H^B}(S) \in (1 \pm \eps)(C_{G^A}(S) + C_{G^A}(S)) = (1 \pm \eps)C_{G}(S).
\]
This means Alice and Bob can exchange $H^A$ and $H^B$ to know $H$. This requires $\tO(n)$-bits of communication, as $H^A$ and $H^B$ has $\tO(n)$ many edges.
\end{proof}


For the formulation of Interval problem, Alice has a set of intervals $\cI^A$ and Bob has another set of interval $\cI^B$. By the same argument as that of Claim \ref{clm:interval-path-eqv}, we can find the equivalence to the problem of finding 2-respecting min-cut where $T$ is a path of length $n$, Alice holds a set of edges corresponding to $\cI^A$ and Bob holds another set of edges corresponding to $\cI^B$. 


\begin{claim}
Line \ref{algline:min-find} of Algorithm \ref{alg:bipartite-int} can be done with $\tilde O(n)$ communication.
\end{claim}

\begin{proof}
Alice can compute $\cost^A(i,{\sf mid})$ for all $i \in L$ and send the column to Bob. This requires $O(n \log n)$ bits of communication. Bob can compute $\cost^B(i,{\sf mid})$ for all $i \in L$ by himself, and add it to Alice's vector to get the actual cost vector. Once done, Bob can find out $i_s$ and $i_t$ and send it to Alice. This requires $O(\log n)$ bits of communication. 
\end{proof}

Now, we can use Claim \ref{clm:interval-gen-comp} to guarantee the communication complexity of the Procedure {\sc Interval}. We have the following corollary.

\begin{corollary} \label{cor:cc-interval}
The communication complexity of Algorithm \ref{alg:int} on a $n$ vertex graph is $\tilde O(n)$
\end{corollary}

At this point, we turn towards the communication complexity of Algorithm \ref{alg:tree}. We start with the following claim:

\begin{claim} \label{clm;cc-pairing}
Alice and Bob can find out the sets $\cP^{cross}_e$ and $\cP^{down}_e$ for every $e \in T$ with $\tilde O(n)$ bits of communication.
\end{claim}

\begin{proof} 
Fix an $e \in T$ and consider any path $p \in \cP^{cross}_e$ which is cross-\interest to $e$. Let $e' \in p$ be the edge closest to the root. Let us also assume that $e$ is the parent edge of vertex $u$ and $e'$ is the parent edge of vertex $v$. This means $C(u^\da, v^\da) > \frac{\deg(u^\da)} 2$. This also implies that at least one of the following is true: $C^A(u^\da, v^\da) > \frac{\deg^A(u^\da)} 2$ or $C^B(u^\da, v^\da) > \frac{\deg^B(u^\da)} 2$. 

Because of Observation \ref{obs:int-vbotv}, \ref{obs:int-ancestor} and Theorem \ref{thm:tree-decomp}, for Alice, there are at most $\log n$ paths $\cP^{cross,A}_e \subseteq \cP$ which are cross-\interest to $e$. This means, for any such path $p^A \in  \cP^{cross,A}_e$ and for $e' \in p^A$ which is closest to the root, $C^A(u^\da, v^\da) > \frac{\deg^A(u^\da)} 2$ (Observation \ref{obs:int-ancestor}). Alice can find the set $\cP^{cross,A}_e$ out by herself. Similarly, for Bob, there are at most $\log n$ many paths $\cP^{cross,B}_e \subseteq \cP$ which are cross-\interest to $u$, \textit{i.e.,} for any such path $p^B \in \cP^{cross,B}_e$, $C^B(u^\da, v'^\da) > \frac{\deg^B(u^\da)} 2$ (where $e''$, which closest to the root in $p^B$, is the parent of $v'$). Bob can find the set $\cP^{cross,B}_e$ out by himself as well. The set of paths which are cross-\interest to $e$ is a subset of $\cP^{cross,A}_e \cup \cP^{cross,B}_e$.

\begin{description}
\item[Step 1: ] Alice and Bob exchange $\deg^A(u^\da)$ and $\deg^B(u^\da)$ for each vertex $u$. This requires $\tilde O(n)$ bits of communication. 
\item[Step 2: ] for each path $p^A \in \cP^{cross,A}_e$ Alice sends to Bob $C^A(u^\da, v^\da)$ where the edge which is closest to the root in $p^A$ is the parent of the vertex $v$. Likewise, for each path $p^B \in \cP^{cross,B}_e$ Bob sends to Alice $C^A(u^\da, v'^\da)$ where the edge which is closest to the root in $p^B$ is the parent of the vertex $v'$.. This requires $O(\log^2 n)$ bits of information for each edge $e$. Hence, in total, $\tilde O(n)$ bits of communication is required.
\end{description}

At this point, Alice and Bob can figure out the set $\cP^{cross}_e$ for each $e$. A similar argument can be made for the case of $\cP^{down}_e$.
\end{proof}

Next, let us try to analyze the communication needed between Alice and Bob to run Algorithm \ref{alg:tree} between themselves. We assume that both Alice and Bob know the spanning tree $T$ and can do the heavy-light decomposition locally without any communication.

\begin{lemma} \label{lem:cc-tworespect}
The 2-party communication complexity of finding a 2-respecting weighted min-cut is $\tilde O(n)$.
\end{lemma}

\begin{proof}
We analyse the communication required between Alice and Bob in each line of Algorithm \ref{alg:tree}.
\begin{description}
\item[Line \ref{algline:1-resp-s} to \ref{algline:1-resp-e}:] For each edge $e$, Alice computes the cut in her graph $G^A$ which respects $e$, and sends the value to Bob. Bob can do the same on $G_B$, and find out the actual cut value by adding these two values. This requires $\log n$ bits of communication per edge of $T$, and hence, $\tilde O(n)$ bits of communication in total.

\item[Line \ref{algline:2-resp-path-s} to \ref{algline:2-resp-path-e}:] Note that the paths in $\cP$ are edge disjoint. Hence each edge takes part in exactly 1 path in $\cP$ and, also, in exactly 1 call to Algorithm \ref{alg:int}. Using Corollary \ref{cor:cc-interval}, we see that the total communication needed is $\tilde O(n)$.

\item[Line \ref{algline:find-interest-s} to \ref{algline:find-interest-e}:] By Claim \ref{clm;cc-pairing}, Alice and Bob needs to communicate at most $\tilde O(n)$ bits.

\item[Line \ref{algline:pairing-s} to \ref{algline:pairing-e}:] We can use Claim \ref{clm:tree-amortize} which says that each edge of $T$ takes part in at most $O(\log n)$ many calls to Algorithm \ref{alg:int}. By Corollary \ref{cor:cc-interval}, the total communication needed is $\tilde O(n)$.
\end{description}
Hence, the total communication required is at most $\tilde O(n)$.
\end{proof}

